Deadlock detection in linear recursive programs

Deadlock detection in recursive programs that admit dynamic resource creation is extremely complex and solutions either give imprecise answers or do not scale. We define an algorithm for detecting deadlocks of "linear recursive programs" of a basic model. The theory that underpins the algorithm is a generalization of the theory of permutations of names to so-called "mutations", which transform tuples by introducing duplicates and fresh names. Our algorithm realizes the back-end of deadlock analyzers for object-oriented programming languages, once the association programs/basic-model-programs has been defined as front-end.

==> mfd-nonlinearcase.tex <==
%

When the lam program is not linear recursive, it is not possible to associate a unique
mutation to a function. In the general case, our technique for verifying 
circularity-freedom consists of 

\smallskip

$\! \! \!\!\!\!\!\!\!\!\bigl( \M'(x,y,z) = (x,y) \sparop \N'(y,z), \;
\N'(x,y) = \N'(x,z) \sparop \M'(z,y,y), \; \P \bigr)$ 

\smallskip

\noindent the recursive
history of $\M'$ is $\M'\N'$.
The sequence $\M'\N'\N'$ \emph{is not} a recursive history
because it contains multiple occurrences of the function $\N'$.
However, if one computes the sequences of invocations 
$\M'(x,y,z) \cdots \M'(\wt{u})$,
it is possible to derive the two sequences $\M'(x,y,z) \N'(y,z) \M'(z',z,z)$
and $\M'(x,y,z) \N'(y,z)$ $\N'(y,u) \M'(u',u,u)$ that define  two different
mutations $\mut{4,3,3}$ and $\mut{6,5,5}$ (see the definition of mutation of a
function). 

the following $\Q'$-program

\smallskip

$\bigl( \Q'(x,y,z) = (x,y) \sparop \Q'(y,z,x) \seq (x,u) \sparop \Q'(u,u,y)
, \; \P \bigr)$ .

\smallskip

In these cases, functions have a unique recursive history
but there are multiple recursive invocations. 
%
On the contrary, the  $\M''\N''$-program below

\smallskip
 
$\begin{array}{ll}
\bigl( \; & \M''(x,y) =  (x,z)\sparop\M''(y,z) \seq \N''(y,x) \; ,
\\
 &\N''(x,y) = (y,x)\sparop\M''(y,z) \sparop \N''(z,x) \;,
 \\
 & \M''(x_1,x_2) \quad
 \bigr)
\end{array}$

\smallskip

For example, the program

\smallskip

$\bigl( \M(x) = (x,y) \sparop \N(x) \; , \; \N(x) = (x,y) \sparop \M(x) \seq \N(y) \; ,   \;\P \; \bigr)$

\smallskip



$\PP''\Q''$-program

\smallskip

$\begin{array}{ll}
\bigl( \; & \PP''(x,y) =  (x,z)\sparop\Q''(y,z) \seq \Q''(y,x) \; ,
\\
 &\Q''(x,y) = (y,x)\sparop\PP''(y,z) \sparop \PP''(z,x) \;,
 \\
 & \PP''(x_1,x_2) \quad
 \bigr)
\end{array}$

\smallskip


For example, the functions $\PP''$ and $\Q''$ in the
$\PP''\Q''$-program are transformed into
 
\smallskip

$\begin{array}{rl}
\PP''(x,y) = &  (x,z)\sparop\Q''(y,z) \seq \Q''(y,x) \; ,
\\
 \Q''(x,y) = & (y,x)\sparop ((y,z')\sparop\Q''(z,z')  \seq \Q''(z,y)) 
 \\
 & \sparop ((z,z'')\sparop\Q''(x,z'') \seq  \Q''(x,z)).
\end{array}$

\smallskip

For example, the $\M''\N''$-program 

\smallskip
 
$\begin{array}{ll}
\bigl( \; & \M''(x,y) =  (x,z)\sparop\M''(y,z) \seq \N''(y,x) \; ,
\\
 &\N''(x,y) = (y,x)\sparop\M''(y,z) \sparop \N''(z,x) \;,
 \\
 & \M''(x_1,x_2) \quad
 \bigr)
\end{array}$

\smallskip

is rewritten into
%

\smallskip 

$\begin{array}{@{\!}ll}
\bigl( & \M''(x,y) =  (x,z)\sparop\N''(x',y',y,z) \seq \N''(y,x,z',z'') \; ,
\\
 &\N''(x,y,u,v) = (y,x)\sparop\M''(y,z) \sparop \N''(z,x,x',y') \sparop \M''(u,v) \;,
 \\
 & \M''(x_1,x_2) \quad
 \bigr) \; .
\end{array}$

\smallskip


%
%
%
%

